A Hybrid Quantum-Classical CFD Methodology with Benchmark HHL Solutions

There has been significant progress in the development of quantum algorithms for solving linear systems of equations with a growing body of applications to Computational Fluid Dynamics (CFD) and CFD-like problems. This work extends previous work by developing a non-linear hybrid quantum-classical CFD solver and using it to generate fully converged solutions. The hybrid solver uses the SIMPLE CFD algorithm, which is common in many industrial CFD codes, and applies it to the 2-dimensional lid driven cavity test case. A theme of this work is the classical processing time needed to prepare the quantum circuit with a focus on the decomposition of the CFD matrix into a linear combination of unitaries (LCU). CFD meshes with up to 65x65 nodes are considered with the largest producing a LCU containing 32,767 Pauli strings. A new method for rapidly re-computing the coefficients in a LCU is proposed, although this reduces, rather than eliminates, the classical scaling issues. The quantum linear equation solver uses the Harrow, Hassidim, Lloyd (HHL) algorithm via a state-vector emulator. Test matrices are sampled from the classical CFD solver to investigate the solution accuracy that can be achieved with HHL. For the smallest 5x5 and 9x9 CFD meshes, full non-linear hybrid CFD calculations are performed. The impacts of approximating the LCU and the varying the number of ancilla rotations in the eigenvalue inversion circuit are studied. Preliminary timing results indicate that the classical computer preparation time needed for a hybrid solver is just as important to the achievement of quantum advantage in CFD as the time on the quantum computer. The reported HHL solutions and LCU decompositions provide a benchmark for future research. The CFD test matrices used in this study are available upon request.

==> references.tex <==
% using Makefile, 4 steps needed when new reference is added, must be cited as well (or after make clean)
% make
% make bib
% make
% make

% -----
%  AAA
% -----
@article{aaronson2015read,
  title={Read the fine print},
  author={Aaronson, Scott},
  journal={Nature Physics},
  volume={11},
  number={4},
  pages={291--293},
  year={2015},
  publisher={Nature Publishing Group}
}

@book{ahokas2004improved,
  title={Improved algorithms for approximate quantum Fourier transforms and sparse Hamiltonian simulations},
  author={Ahokas, Graeme Robert},
  year={2004},
  publisher={University of Calgary}
}

@article{ammour2018subgrid,
  title={The Subgrid-Scale Approach for Modeling Impingement Cooling Flow in the Combustor Pedestal Tile},
  author={Ammour, Dalila and Page, Gary J},
  journal={Journal of Heat Transfer},
  volume={140},
  number={4},
  year={2018},
  publisher={American Society of Mechanical Engineers Digital Collection}
}

@article{araujo2021divide,
  title={A divide-and-conquer algorithm for quantum state preparation},
  author={Araujo, Israel F and Park, Daniel K and Petruccione, Francesco and da Silva, Adenilton J},
  journal={Scientific Reports},
  volume={11},
  number={1},
  pages={1--12},
  year={2021},
  publisher={Nature Publishing Group}
}

% -----
%  BBB
% -----
@article{babbush2018encoding,
  title={Encoding electronic spectra in quantum circuits with linear T complexity},
  author={Babbush, Ryan and Gidney, Craig and Berry, Dominic W and Wiebe, Nathan and McClean, Jarrod and Paler, Alexandru and Fowler, Austin and Neven, Hartmut},
  journal={Physical Review X},
  volume={8},
  number={4},
  pages={041015},
  year={2018},
  publisher={APS}
}

@article{barenco1995elementary,
  title={Elementary gates for quantum computation},
  author={Barenco, Adriano and Bennett, Charles H and Cleve, Richard and DiVincenzo, David P and Margolus, Norman and Shor, Peter and Sleator, Tycho and Smolin, John A and Weinfurter, Harald},
  journal={Physical review A},
  volume={52},
  number={5},
  pages={3457},
  year={1995},
  publisher={APS}
}

@article{berry2007efficient,
  title={Efficient quantum algorithms for simulating sparse Hamiltonians},
  author={Berry, Dominic W and Ahokas, Graeme and Cleve, Richard and Sanders, Barry C},
  journal={Communications in Mathematical Physics},
  volume={270},
  number={2},
  pages={359--371},
  year={2007},
  publisher={Springer}
}

@article{berry2015simulating,
  title={Simulating Hamiltonian dynamics with a truncated Taylor series},
  author={Berry, Dominic W and Childs, Andrew M and Cleve, Richard and Kothari, Robin and Somma, Rolando D},
  journal={Physical review letters},
  volume={114},
  number={9},
  pages={090502},
  year={2015},
  publisher={APS}
}

@article{berry2018improved,
  title={Improved techniques for preparing eigenstates of fermionic Hamiltonians},
  author={Berry, Dominic W and Kieferov{\'a}, M{\'a}ria and Scherer, Artur and Sanders, Yuval R and Low, Guang Hao and Wiebe, Nathan and Gidney, Craig and Babbush, Ryan},
  journal={npj Quantum Information},
  volume={4},
  number={1},
  pages={1--7},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{blais2020lethe,
  title={Lethe: An open-source parallel high-order adaptative CFD solver for incompressible flows},
  author={Blais, Bruno and Barbeau, Lucka and Bibeau, Val{\'e}rie and Gauvin, Simon and El Geitani, Toni and Golshan, Shahab and Kamble, Rajeshwari and Mirakhori, Ghazaleh and Chaouki, Jamal},
  journal={SoftwareX},
  volume={12},
  pages={100579},
  year={2020},
  publisher={Elsevier}
}

@article{bouffanais2007large,
  title={Large-eddy simulation of the flow in a lid-driven cubical cavity},
  author={Bouffanais, Roland and Deville, Michel O and Leriche, Emmanuel},
  journal={Physics of Fluids},
  volume={19},
  number={5},
  pages={055108},
  year={2007},
  publisher={American Institute of Physics}
}

@article{bravyi2021simulate,
  title={How to simulate quantum measurement without computing marginals},
  author={Bravyi, Sergey and Gosset, David and Liu, Yinchen},
  journal={arXiv preprint arXiv:2112.08499},
  year={2021}
}

@article{ljubomir2022quantum,
  title={Quantum algorithm for the Navier--Stokes equations by using the streamfunction-vorticity formulation and the lattice Boltzmann method},
  author={Ljubomir, Budinski},
  journal={International Journal of Quantum Information},
  pages={2150039},
  year={2022},
  publisher={World Scientific}
}

% -----
%  CCC
% -----
@article{camps2022explicit,
  title={Explicit Quantum Circuits for Block Encodings of Certain Sparse Matrice},
  author={Camps, Daan and Lin, Lin and Van Beeumen, Roel and Yang, Chao},
  journal={arXiv preprint arXiv:2203.10236},
  year={2022}
}

@article{cao2012quantum,
  title={Quantum circuit design for solving linear systems of equations},
  author={Cao, Yudong and Daskin, Anmer and Frankel, Steven and Kais, Sabre},
  journal={Molecular Physics},
  volume={110},
  number={15-16},
  pages={1675--1680},
  year={2012},
  publisher={Taylor \& Francis}
}

@article{cao2013quantum,
  title={Quantum circuits for solving linear systems of equations},
  author={Cao, Yudong and Daskin, Anmer and Frankel, Steven and Kais, Sabre},
  journal={arXiv preprint arXiv:1110.2232v3},
  year={2013}
}

@article{cao2013quantum2,
  title={Quantum algorithm and circuit design solving the Poisson equation},
  author={Cao, Yudong and Papageorgiou, Anargyros and Petras, Iasonas and Traub, Joseph and Kais, Sabre},
  journal={New Journal of Physics},
  volume={15},
  number={1},
  pages={013021},
  year={2013},
  publisher={IOP Publishing}
}

@misc{qasm2circ,
  title        = {Quantum Circuit Viewer: qasm2circ, Massachusetts Institute of Technology},
  author       = {Chuang, I},
  howpublished = {\url{https://www.media.mit.edu/quanta/qasm2circ/}},
  year         = 2005,
  note         = "Accessed: 2020-12-05"
}

@inproceedings{childs2010simulating,
  title={Simulating sparse Hamiltonians with star decompositions},
  author={Childs, Andrew M and Kothari, Robin},
  booktitle={Conference on Quantum Computation, Communication, and Cryptography},
  pages={94--103},
  year={2010},
  organization={Springer}
}

@article{childs2012hamiltonian,
  title={Hamiltonian simulation using linear combinations of unitary operations},
  author={Childs, Andrew M and Wiebe, Nathan},
  journal={arXiv preprint arXiv:1202.5822},
  year={2012}
}

@article{cohen1982eigenvalue,
  title={Eigenvalue inequalities for products of matrix exponentials},
  author={Cohen, Joel E and Friedland, Shmuel and Kato, Tosio and Kelly, Frank P},
  journal={Linear Algebra and its Applications},
  volume={45},
  pages={55--95},
  year={1982},
  publisher={Elsevier}
}

@article{costa2019quantum,
  title={Quantum algorithm for simulating the wave equation},
  author={Costa, Pedro CS and Jordan, Stephen and Ostrander, Aaron},
  journal={Physical Review A},
  volume={99},
  number={1},
  pages={012323},
  year={2019},
  publisher={APS}
}

@article{courbebaisse2011time,
  title={Time-scale joint representation of DNS and LES numerical data},
  author={Courbebaisse, Guy and Bouffanais, Roland and Navarro, Laurent and Leriche, Emmanuel and Deville, Michel},
  journal={Computers \& fluids},
  volume={43},
  number={1},
  pages={38--45},
  year={2011},
  publisher={Elsevier}
}

% -----
%  DDD
% -----
@proceedings{10.1115/82-GT-239,
    author = {Denton, J. D.},
    title = "{An Improved Time Marching Method for Turbomachinery Flow Calculation}",
    volume = {Volume 1: Turbomachinery},
    series = {Turbo Expo: Power for Land, Sea, and Air},
    year = {1982},
    month = {04},
    abstract = "{Time marching solutions of the Euler equations are now very widely used for the calculation of flow through turbomachinery blade rows. All methods suffer from the disadvantages of shock smearing, lack of entropy conservation, and comparatively long run times. A new method is described which reduces all these problems. The method is based on the author’s opposed difference scheme, but this is applied to a new type of grid consisting of quadrilateral elements which do not overlap and have nodes only at their corners. The use of a nonoverlapping grid reduces finite differencing errors and gives complete freedom to vary the size of the elements. Both these factors help to improve entropy conservation. Considerable savings in run time (by a factor of about 3) are obtained by using a simple multigrid method whereby the solution is advanced simultaneously on a course and on a fine grid. The resulting method is simpler, faster, and more accurate than its predecessor.}",
    doi = {10.1115/82-GT-239},
    url = {https://doi.org/10.1115/82-GT-239},
    note = {V001T01A082},
    eprint = {https://asmedigitalcollection.asme.org/GT/proceedings-pdf/GT1982/79566/V001T01A082/2394030/v001t01a082-82-gt-239.pdf},
}

@article{dervovic2018quantum,
  title={Quantum linear systems algorithms: a primer},
  author={Dervovic, Danial and Herbster, Mark and Mountney, Peter and Severini, Simone and Usher, Na{\"\i}ri and Wossnig, Leonard},
  journal={arXiv preprint arXiv:1802.08227},
  year={2018}
}

@article{de2020decomposition,
  title={The decomposition of an arbitrary 2w$\times$ 2w unitary matrix into signed permutation matrices},
  author={De Vos, Alexis and De Baerdemacker, Stijn},
  journal={Linear Algebra and its Applications},
  volume={606},
  pages={23--40},
  year={2020},
  publisher={Elsevier}
}

@article{dong2021efficient,
  title={Efficient phase-factor evaluation in quantum signal processing},
  author={Dong, Yulong and Meng, Xiang and Whaley, K Birgitta and Lin, Lin},
  journal={Physical Review A},
  volume={103},
  number={4},
  pages={042419},
  year={2021},
  publisher={APS}
}
@article{dong2021quantum,
  title={A Quantum Hamiltonian Simulation Benchmark},
  author={Dong, Yulong and Whaley, K Birgitta and Lin, Lin},
  journal={arXiv preprint arXiv:2108.03747},
  year={2021}
}

@article{dong2021random,
  title={Random circuit block-encoded matrix and a proposal of quantum LINPACK benchmark},
  author={Dong, Yulong and Lin, Lin},
  journal={Physical Review A},
  volume={103},
  number={6},
  pages={062412},
  year={2021},
  publisher={APS}
}

@article{doronin2020solving,
  title={Solving systems of linear algebraic equations via unitary transformations on quantum processor of IBM Quantum Experience},
  author={Doronin, Sergey I and Fel’dman, EB and Zenchuk, Alexandre I},
  journal={Quantum Information Processing},
  volume={19},
  number={2},
  pages={1--20},
  year={2020},
  publisher={Springer}
}

@misc{draper2017qpic,
  title={QPIC: Quantum circuit diagrams in latex},
  author={Draper, Thomas and Kutin, Samuel},
  howpublished = {\url{https://github.com/qpic/qpic/blob/master/doc/qpic_doc.pdf}},
  year={2017}
}

@article{duan2020survey,
  title={A survey on HHL algorithm: From theory to application in quantum machine learning},
  author={Duan, Bojia and Yuan, Jiabin and Yu, Chao-Hua and Huang, Jianbang and Hsieh, Chang-Yu},
  journal={Physics Letters A},
  volume={384},
  number={24},
  pages={126595},
  year={2020},
  publisher={Elsevier}
}

@article{dutta2020quantum,
  title={Quantum circuit design methodology for multiple linear regression},
  author={Dutta, Sanchayan and Suau, Adrien and Dutta, Sagnik and Roy, Suvadeep and Behera, Bikash K and Panigrahi, Prasanta K},
  journal={IET Quantum Communication},
  volume={1},
  number={2},
  pages={55--61},
  year={2020},
  publisher={Wiley Online Library}
}

% -----
%  FFF
% -----
@article{fontanela2019quantum,
  title={A Quantum algorithm for linear PDEs arising in Finance},
  author={Fontanela, Filipe and Jacquier, Antoine Jack and Oumgari, Mugad},
  journal={Available at SSRN 3499134},
  year={2019}
}

% -----
%  GGG
% -----
@article{gaitan2020finding,
  title={Finding flows of a Navier--Stokes fluid through quantum computing},
  author={Gaitan, Frank},
  journal={npj Quantum Information},
  volume={6},
  number={1},
  pages={1--6},
  year={2020},
  publisher={Nature Publishing Group}
}

@incollection{gerstenberger20213d,
  title={3D CFD In-situ Co-processing for Turbomachinery Design},
  author={Gerstenberger, Axel},
  booktitle={ISAV'21: In Situ Infrastructures for Enabling Extreme-Scale Analysis and Visualization},
  year={2021}
}

@inproceedings{ghia1977study,
  title={Study of incompressible Navier-Stokes equations in primitive variables using implicit numerical technique},
  author={Ghia, K and Hankey, JR, W and Hodge, J},
  booktitle={3rd Computational Fluid Dynamics Conference},
  pages={648},
  year={1977}
}

@article{ghia1982high,
  title={High-Re solutions for incompressible flow using the Navier-Stokes equations and a multigrid method},
  author={Ghia, UKNG and Ghia, Kirti N and Shin, CT},
  journal={Journal of computational physics},
  volume={48},
  number={3},
  pages={387--411},
  year={1982},
  publisher={Elsevier}
}

@inproceedings{gilyen2019quantum,
  title={Quantum singular value transformation and beyond: exponential improvements for quantum matrix arithmetics},
  author={Gily{\'e}n, Andr{\'a}s and Su, Yuan and Low, Guang Hao and Wiebe, Nathan},
  booktitle={Proceedings of the 51st Annual ACM SIGACT Symposium on Theory of Computing},
  pages={193--204},
  year={2019}
}

@article{givi2020quantum,
  title={Quantum speedup for aeroscience and engineering},
  author={Givi, Peyman and Daley, Andrew J and Mavriplis, Dimitri and Malik, Mujeeb},
  journal={AIAA Journal},
  volume={58},
  number={8},
  pages={3715--3727},
  year={2020},
  publisher={American Institute of Aeronautics and Astronautics}
}

@book{gough2009gnu,
  title={GNU scientific library reference manual},
  author={Gough, Brian},
  year={2009},
  publisher={Network Theory Ltd.}
}

% -----
%  HHH
% -----
@article{harlow1965numerical,
  title={Numerical calculation of time-dependent viscous incompressible flow of fluid with free surface},
  author={Harlow, Francis H and Welch, J Eddie},
  journal={The physics of fluids},
  volume={8},
  number={12},
  pages={2182--2189},
  year={1965},
  publisher={American Institute of Physics}
}

@article{harrow2009quantum,
  title={Quantum algorithm for linear systems of equations},
  author={Harrow, Aram W and Hassidim, Avinatan and Lloyd, Seth},
  journal={Physical review letters},
  volume={103},
  number={15},
  pages={150502},
  year={2009},
  publisher={APS}
}

@article{hills2007achieving,
  title={Achieving high parallel performance for an unstructured unsteady turbomachinery CFD code},
  author={Hills, N},
  journal={The aeronautical journal},
  volume={111},
  number={1117},
  pages={185--193},
  year={2007},
  publisher={Cambridge University Press}
}

@inproceedings{humble2018simulated,
  title={Simulated execution of hybrid quantum computing systems},
  author={Humble, Travis S and Sadlier, Ronald J and Britt, Keith A},
  booktitle={Quantum Information Science, Sensing, and Computation X},
  volume={10660},
  pages={1066002},
  year={2018},
  organization={International Society for Optics and Photonics}
}

% -----
%  JJJ
% -----
@misc{nlopt,
  title        = {The {NL}opt nonlinear-optimization package},
  author       = {Johnson, Steven G},
  howpublished = {\url{http://github.com/stevengj/nlopt}},
  year         = 2020,
}

@book{johnston2019programming,
  title={Programming Quantum Computers: essential algorithms and code samples},
  author={Johnston, Eric R and Harrigan, Nic and Gimeno-Segovia, Mercedes},
  year={2019},
  publisher={" O'Reilly Media, Inc."}
}

@article{jones2019quest,
  title={QuEST and high performance simulation of quantum computers},
  author={Jones, Tyson and Brown, Anna and Bush, Ian and Benjamin, Simon C},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={1--11},
  year={2019},
  publisher={Nature Publishing Group}
}

% -----
%  KKK
% -----
@article{kacewicz2006almost,
  title={Almost optimal solution of initial-value problems by randomized and quantum algorithms},
  author={Kacewicz, Boles{\l}aw},
  journal={Journal of Complexity},
  volume={22},
  number={5},
  pages={676--690},
  year={2006},
  publisher={Elsevier}
}

@mastersthesis{kothari2010efficient,
  title={Efficient simulation of Hamiltonians},
  author={Kothari, Robin},
  year={2010},
  school={University of Waterloo}
}

@phdthesis{kothari2014efficient,
  title={Efficient algorithms in quantum query complexity},
  author={Kothari, Robin},
  year={2014},
  school={University of Waterloo},
  url = {https://uwspace.uwaterloo.ca/handle/10012/8625}
}

@article{kulkarni1999eigenvalues,
  title={Eigenvalues of tridiagonal pseudo-Toeplitz matrices},
  author={Kulkarni, Devadatta and Schmidt, Darrell and Tsui, Sze-Kai},
  journal={Linear Algebra and its Applications},
  volume={297},
  pages={63--80},
  year={1999}
}

@article{kyriienko2021solving,
  title={Solving nonlinear differential equations with differentiable quantum circuits},
  author={Kyriienko, Oleksandr and Paine, Annie E and Elfving, Vincent E},
  journal={Physical Review A},
  volume={103},
  number={5},
  pages={052416},
  year={2021},
  publisher={APS}
}

% -----
%  LLL
% -----
@inproceedings{lapworth2003bypass,
  title={Challenges and Methodologies in the Design of Axial Flow Fans for High Bypass Ratio Gas Turbine Engines Using Steady and Unsteady {CFD}},
  author={Lapworth, L},
  booktitle={Advances of CFD in fluid machinery design},
  editor={Robin Elder, Antonios Tourlidakis, Martin Yates},
  year={2003},
  publisher={John Wiley \& Sons}
}

@article{lapworth2021parallel,
  title={Parallel encryption of input and output data for HPC applications},
  author={Lapworth, Leigh},
  journal={The International Journal of High Performance Computing Applications},
  pages={10943420211016516},
  year={2021},
  publisher={SAGE Publications Sage UK: London, England}
}

@misc{lapworth2022patent,
  title        = {Determining Solutions to a Number of Linear Matrix Equations},
  author       = {Lapworth, L},
  note         = "Patent Application GB2207665.7, filed 25 May 2022."
}

@inproceedings{neittaanmaki2004design,
  title={Design of Gas Turbine Engines using {CFD}},
  author={Lapworth, B L and Shahpar, S},
  booktitle={European Congress on Computational Methods in Applied Sciences and Engineering (ECCOMAS)},
  editor={Neittaanm{\"a}ki, P and Rossi, T and Korotov, S and Onate, E and P{\'e}riaux, J and Kn{\"o}rzer, D},
  year={2004}
}

@article{lee2019hybrid,
  title={Hybrid quantum linear equation algorithm and its experimental test on ibm quantum experience},
  author={Lee, Yonghae and Joo, Jaewoo and Lee, Soojoon},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={1--12},
  year={2019},
  publisher={Nature Publishing Group}
}

@inproceedings{li2021sv,
  title={SV-sim: scalable PGAS-based state vector simulation of quantum circuits},
  author={Li, Ang and Fang, Bo and Granade, Christopher and Prawiroatmodjo, Guen and Heim, Bettina and Roetteler, Martin and Krishnamoorthy, Sriram},
  booktitle={Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
  pages={1--14},
  year={2021}
}

@article{Low2019hamiltonian,
  doi = {10.22331/q-2019-07-12-163},
  url = {https://doi.org/10.22331/q-2019-07-12-163},
  title = {Hamiltonian {S}imulation by {Q}ubitization},
  author = {Low, Guang Hao and Chuang, Isaac L.},
  journal = {{Quantum}},
  issn = {2521-327X},
  publisher = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
  volume = {3},
  pages = {163},
  month = jul,
  year = {2019}
}

@inproceedings{lu2020quantum,
  title={Quantum CFD simulations for heat transfer applications},
  author={Lu, Chao and Hu, Zhao and Xie, Bei and Zhang, Ning},
  booktitle={ASME International Mechanical Engineering Congress and Exposition},
  volume={84584},
  pages={V010T10A050},
  year={2020},
  organization={American Society of Mechanical Engineers}
}

@article{lubasch2020variational,
  title={Variational quantum algorithms for nonlinear problems},
  author={Lubasch, Michael and Joo, Jaewoo and Moinier, Pierre and Kiffner, Martin and Jaksch, Dieter},
  journal={Physical Review A},
  volume={101},
  number={1},
  pages={010301},
  year={2020},
  publisher={APS}
}

% -----
%  MMM
% -----
@article{martyn2021grand,
  title={Grand unification of quantum algorithms},
  author={Martyn, John M and Rossi, Zane M and Tan, Andrew K and Chuang, Isaac L},
  journal={PRX Quantum},
  volume={2},
  number={4},
  pages={040203},
  year={2021},
  publisher={APS}
}

@article{mazhar2016novel,
  title={A novel fully implicit block coupled solution strategy for the ultimate treatment of the velocity--pressure coupling problem in incompressible fluid flow},
  author={Mazhar, Zeka},
  journal={Numerical Heat Transfer, Part B: Fundamentals},
  volume={69},
  number={2},
  pages={130--149},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{mcclean2016theory,
  title={The theory of variational hybrid quantum-classical algorithms},
  author={McClean, Jarrod R and Romero, Jonathan and Babbush, Ryan and Aspuru-Guzik, Al{\'a}n},
  journal={New Journal of Physics},
  volume={18},
  number={2},
  pages={023023},
  year={2016},
  publisher={IOP Publishing}
}

@article{mcguirk1990shock,
  title={Shock capturing using a pressure-correction method},
  author={McGuirk, James J and Page, Gary J},
  journal={AIAA journal},
  volume={28},
  number={10},
  pages={1751--1757},
  year={1990}
}

@misc{minato_vqe,
  title        = {Variational Quantum Eigensolver and {QAOA} Introduction},
  author       = {Yuichiro Minato},
  howpublished = {\url{https://medium.com/mdr-inc/variational-quantum-eigensolver-qaoa-introduction-9e6c8e19d9cb}},
  year         = 2020,
  note         = "Accessed: 2020-11-06"
}

@article{mottonen2004transformation,
  title={Transformation of quantum states using uniformly controlled rotations},
  author={Mottonen, Mikko and Vartiainen, Juha J and Bergholm, Ville and Salomaa, Martti M},
  journal={arXiv preprint quant-ph/0407010},
  year={2004}
}

% -----
%  NNN
% -----
@article{nannicini2020introduction,
  title={An introduction to quantum computing, without the physics},
  author={Nannicini, Giacomo},
  journal={SIAM Review},
  volume={62},
  number={4},
  pages={936--981},
  year={2020},
  publisher={SIAM}
}

@article{ni1982multiple,
  title={A multiple-grid scheme for solving the Euler equations},
  author={Ni, Ron-Ho},
  journal={AIAA journal},
  volume={20},
  number={11},
  pages={1565--1571},
  year={1982}
}

@article{nielsen2005fermionic,
  title={The Fermionic canonical commutation relations and the Jordan-Wigner transform},
  author={Nielsen, Michael A and others},
  journal={School of Physical Sciences The University of Queensland},
  volume={59},
  year={2005}
}

@misc{nielsen2002quantum,
  title={Quantum computation and quantum information},
  author={Nielsen, Michael A and Chuang, Isaac},
  year={2000},
  publisher={Cambridge University Press, Cambridge, United Kingdom}
}

% -----
%  OOO
% -----

% -----
%  PPP
% -----
@article{pan2014experimental,
  title={Experimental realization of quantum algorithm for solving linear systems of equations},
  author={Pan, Jian and Cao, Yudong and Yao, Xiwei and Li, Zhaokai and Ju, Chenyong and Chen, Hongwei and Peng, Xinhua and Kais, Sabre and Du, Jiangfeng},
  journal={Physical Review A},
  volume={89},
  number={2},
  pages={022313},
  year={2014},
  publisher={APS}
}

@article{patankar1972calculation,
  title={A calculation procedure for heat, mass and momentum transfer in three-dimensional parabolic flows},
  author={Patankar, SV and Spalding, DB},
  journal={Int. J. Heat Mass Transfer},
  volume={15},
  pages={1787--1806},
  year={1972},
}

@article{patankar1975prediction,
  title={Prediction of turbulent flow in curved pipes},
  author={Patankar, Suhas V and Pratap, VS and Spalding, DB},
  journal={Journal of Fluid Mechanics},
  volume={67},
  number={3},
  pages={583--595},
  year={1975},
  publisher={Cambridge University Press}
}

@inproceedings{perez2020large,
  title={Large-eddy simulation of an integrated high-pressure compressor and combustion chamber of a typical turbine engine architecture},
  author={P{\'e}rez Arroyo, Carlos and Dombard, J{\'e}r{\^o}me and Duchaine, Florent and Gicquel, Laurent and Odier, Nicolas and Exilard, Gorka and Richard, St{\'e}phane and Buffaz, Nicolas and D{\'e}molis, Jacques},
  booktitle={Turbo Expo: Power for Land, Sea, and Air},
  volume={84089},
  pages={V02CT35A058},
  year={2020},
  organization={American Society of Mechanical Engineers}
}

@article{peruzzo2013variational,
  title={A variational eigenvalue solver on a quantum processor. eprint},
  author={Peruzzo, A and others},
  journal={arXiv preprint arXiv:1304.3061},
  year={2013}
}

@article{powell2009bobyqa,
  title={The BOBYQA algorithm for bound constrained optimization without derivatives},
  author={Powell, Michael JD},
  journal={Cambridge NA Report NA2009/06, University of Cambridge, Cambridge},
  pages={26--46},
  year={2009}
}

@inproceedings{puyero1997efficient,
  title={An efficient Newton-GMRES solver for aerodynamic computations},
  author={Puyero, Alberto and Zingg, David and Puyero, Alberto and Zingg, David},
  booktitle={13th Computational Fluid Dynamics Conference},
  pages={1955},
  year={1997}
}

% -----
%  QQQ
% -----
@misc{Qiskit,
       author = {MD SAJID ANIS and Abby-Mitchell and H{\'e}ctor Abraham and AduOffei and Rochisha Agarwal and Gabriele Agliardi and Merav Aharoni and Ismail Yunus Akhalwaya and Gadi Aleksandrowicz and Thomas Alexander and Matthew Amy and Sashwat Anagolum and Eli Arbel and Abraham Asfaw and Anish Athalye and Artur Avkhadiev and Carlos Azaustre and PRATHAMESH BHOLE and Abhik Banerjee and Santanu Banerjee and Will Bang and Aman Bansal and Panagiotis Barkoutsos and Ashish Barnawal and George Barron and George S. Barron and Luciano Bello and Yael Ben-Haim and M. Chandler Bennett and Daniel Bevenius and Dhruv Bhatnagar and Arjun Bhobe and Paolo Bianchini and Lev S. Bishop and Carsten Blank and Sorin Bolos and Soham Bopardikar and Samuel Bosch and Sebastian Brandhofer and Brandon and Sergey Bravyi and Nick Bronn and Bryce-Fuller and David Bucher and Artemiy Burov and Fran Cabrera and Padraic Calpin and Lauren Capelluto and Jorge Carballo and Gin{\'e}s Carrascal and Adam Carriker and Ivan Carvalho and Adrian Chen and Chun-Fu Chen and Edward Chen and Jielun (Chris) Chen and Richard Chen and Franck Chevallier and Kartik Chinda and Rathish Cholarajan and Jerry M. Chow and Spencer Churchill and CisterMoke and Christian Claus and Christian Clauss and Caleb Clothier and Romilly Cocking and Ryan Cocuzzo and Jordan Connor and Filipe Correa and Zachary Crockett and Abigail J. Cross and Andrew W. Cross and Simon Cross and Juan Cruz-Benito and Chris Culver and Antonio D. C{\'o}rcoles-Gonzales and Navaneeth D and Sean Dague and Tareq El Dandachi and Animesh N Dangwal and Jonathan Daniel and Marcus Daniels and Matthieu Dartiailh and Abd{\'o}n Rodr{\'\i}guez Davila and Faisal Debouni and Anton Dekusar and Amol Deshmukh and Mohit Deshpande and Delton Ding and Jun Doi and Eli M. Dow and Eric Drechsler and Eugene Dumitrescu and Karel Dumon and Ivan Duran and Kareem EL-Safty and Eric Eastman and Grant Eberle and Amir Ebrahimi and Pieter Eendebak and Daniel Egger and ElePT and Emilio and Alberto Espiricueta and Mark Everitt and Davide Facoetti and Farida and Paco Mart{\'\i}n Fern{\'a}ndez and Samuele Ferracin and Davide Ferrari and Axel Hern{\'a}ndez Ferrera and Romain Fouilland and Albert Frisch and Andreas Fuhrer and Bryce Fuller and MELVIN GEORGE and Julien Gacon and Borja Godoy Gago and Claudio Gambella and Jay M. Gambetta and Adhisha Gammanpila and Luis Garcia and Tanya Garg and Shelly Garion and James R. Garrison and Tim Gates and Leron Gil and Austin Gilliam and Aditya Giridharan and Juan Gomez-Mosquera and Gonzalo and Salvador de la Puente Gonz{\'a}lez and Jesse Gorzinski and Ian Gould and Donny Greenberg and Dmitry Grinko and Wen Guan and Dani Guijo and John A. Gunnels and Harshit Gupta and Naman Gupta and Jakob M. G{\"u}nther and Mikael Haglund and Isabel Haide and Ikko Hamamura and Omar Costa Hamido and Frank Harkins and Kevin Hartman and Areeq Hasan and Vojtech Havlicek and Joe Hellmers and {\L}ukasz Herok and Stefan Hillmich and Hiroshi Horii and Connor Howington and Shaohan Hu and Wei Hu and Junye Huang and Rolf Huisman and Haruki Imai and Takashi Imamichi and Kazuaki Ishizaki and Ishwor and Raban Iten and Toshinari Itoko and Alexander Ivrii and Ali Javadi and Ali Javadi-Abhari and Wahaj Javed and Qian Jianhua and Madhav Jivrajani and Kiran Johns and Scott Johnstun and Jonathan-Shoemaker and JosDenmark and JoshDumo and John Judge and Tal Kachmann and Akshay Kale and Naoki Kanazawa and Jessica Kane and Kang-Bae and Annanay Kapila and Anton Karazeev and Paul Kassebaum and Josh Kelso and Scott Kelso and Vismai Khanderao and Spencer King and Yuri Kobayashi and Kovi11Day and Arseny Kovyrshin and Rajiv Krishnakumar and Vivek Krishnan and Kevin Krsulich and Prasad Kumkar and Gawel Kus and Ryan LaRose and Enrique Lacal and Rapha{\"e}l Lambert and Haggai Landa and John Lapeyre and Joe Latone and Scott Lawrence and Christina Lee and Gushu Li and Jake Lishman and Dennis Liu and Peng Liu and Lolcroc and Abhishek K M and Liam Madden and Yunho Maeng and Saurav Maheshkar and Kahan Majmudar and Aleksei Malyshev and Mohamed El Mandouh and Joshua Manela and Manjula and Jakub Marecek and Manoel Marques and Kunal Marwaha and Dmitri Maslov and Pawe{\l} Maszota and Dolph Mathews and Atsushi Matsuo and Farai Mazhandu and Doug McClure and Maureen McElaney and Cameron McGarry and David McKay and Dan McPherson and Srujan Meesala and Dekel Meirom and Corey Mendell and Thomas Metcalfe and Martin Mevissen and Andrew Meyer and Antonio Mezzacapo and Rohit Midha and Daniel Miller and Zlatko Minev and Abby Mitchell and Nikolaj Moll and Alejandro Montanez and Gabriel Monteiro and Michael Duane Mooring and Renier Morales and Niall Moran and David Morcuende and Seif Mostafa and Mario Motta and Romain Moyard and Prakash Murali and Jan M{\"u}ggenburg and Tristan NEMOZ and David Nadlinger and Ken Nakanishi and Giacomo Nannicini and Paul Nation and Edwin Navarro and Yehuda Naveh and Scott Wyman Neagle and Patrick Neuweiler and Aziz Ngoueya and Johan Nicander and Nick-Singstock and Pradeep Niroula and Hassi Norlen and NuoWenLei and Lee James O'Riordan and Oluwatobi Ogunbayo and Pauline Ollitrault and Tamiya Onodera and Raul Otaolea and Steven Oud and Dan Padilha and Hanhee Paik and Soham Pal and Yuchen Pang and Ashish Panigrahi and Vincent R. Pascuzzi and Simone Perriello and Eric Peterson and Anna Phan and Kuba Pilch and Francesco Piro and Marco Pistoia and Christophe Piveteau and Julia Plewa and Pierre Pocreau and Alejandro Pozas-Kerstjens and Rafa{\l} Pracht and Milos Prokop and Viktor Prutyanov and Sumit Puri and Daniel Puzzuoli and Jes{\'u}s P{\'e}rez and Quant02 and Quintiii and Rafey Iqbal Rahman and Arun Raja and Roshan Rajeev and Isha Rajput and Nipun Ramagiri and Anirudh Rao and Rudy Raymond and Oliver Reardon-Smith and Rafael Mart{\'\i}n-Cuevas Redondo and Max Reuter and Julia Rice and Matt Riedemann and Rietesh and Drew Risinger and Marcello La Rocca and Diego M. Rodr{\'\i}guez and RohithKarur and Ben Rosand and Max Rossmannek and Mingi Ryu and Tharrmashastha SAPV and Nahum Rosa Cruz Sa and Arijit Saha and Abdullah Ash- Saki and Sankalp Sanand and Martin Sandberg and Hirmay Sandesara and Ritvik Sapra and Hayk Sargsyan and Aniruddha Sarkar and Ninad Sathaye and Bruno Schmitt and Chris Schnabel and Zachary Schoenfeld and Travis L. Scholten and Eddie Schoute and Mark Schulterbrandt and Joachim Schwarm and James Seaward and Sergi and Ismael Faro Sertage and Kanav Setia and Freya Shah and Nathan Shammah and Rohan Sharma and Yunong Shi and Jonathan Shoemaker and Adenilton Silva and Andrea Simonetto and Deeksha Singh and Divyanshu Singh and Parmeet Singh and Phattharaporn Singkanipa and Yukio Siraichi and Siri and Jes{\'u}s Sistos and Iskandar Sitdikov and Seyon Sivarajah and Magnus Berg Sletfjerding and John A. Smolin and Mathias Soeken and Igor Olegovich Sokolov and Igor Sokolov and Vicente P. Soloviev and SooluThomas and Starfish and Dominik Steenken and Matt Stypulkoski and Adrien Suau and Shaojun Sun and Kevin J. Sung and Makoto Suwama and Oskar S{\l}owik and Hitomi Takahashi and Tanvesh Takawale and Ivano Tavernelli and Charles Taylor and Pete Taylour and Soolu Thomas and Kevin Tian and Mathieu Tillet and Maddy Tod and Miroslav Tomasik and Caroline Tornow and Enrique de la Torre and Juan Luis S{\'a}nchez Toural and Kenso Trabing and Matthew Treinish and Dimitar Trenev and TrishaPe and Felix Truger and Georgios Tsilimigkounakis and Davindra Tulsi and Wes Turner and Yotam Vaknin and Carmen Recio Valcarce and Francois Varchon and Adish Vartak and Almudena Carrera Vazquez and Prajjwal Vijaywargiya and Victor Villar and Bhargav Vishnu and Desiree Vogt-Lee and Christophe Vuillot and James Weaver and Johannes Weidenfeller and Rafal Wieczorek and Jonathan A. Wildstrom and Jessica Wilson and Erick Winston and WinterSoldier and Jack J. Woehr and Stefan Woerner and Ryan Woo and Christopher J. Wood and Ryan Wood and Steve Wood and James Wootton and Matt Wright and Lucy Xing and Jintao YU and Bo Yang and Unchun Yang and Jimmy Yao and Daniyar Yeralin and Ryota Yonekura and David Yonge-Mallo and Ryuhei Yoshida and Richard Young and Jessie Yu and Lebin Yu and Christopher Zachow and Laura Zdanski and Helena Zhang and Iulia Zidaru and Christa Zoufal and aeddins-ibm and alexzhang13 and b63 and bartek-bartlomiej and bcamorrison and brandhsn and charmerDark and deeplokhande and dekel.meirom and dime10 and dlasecki and ehchen and fanizzamarco and fs1132429 and gadial and galeinston and georgezhou20 and georgios-ts and gruu and hhorii and hykavitha and itoko and jeppevinkel and jessica-angel7 and jezerjojo14 and jliu45 and jscott2 and klinvill and krutik2966 and ma5x and michelle4654 and msuwama and nico-lgrs and ntgiwsvp and ordmoj and sagar pahwa and pritamsinha2304 and ryancocuzzo and saswati-qiskit and septembrr and sethmerkel and sg495 and shaashwat and sternparky and strickroman and tigerjack and tsura-crisaldo and vadebayo49 and welien and willhbang and wmurphy-collabstar and yang.luh and Mantas {\v{C}}epulkovskis},
       title = {Qiskit: An Open-source Framework for Quantum Computing},
       year = {2021},
       doi = {10.5281/zenodo.2573505}
}

% -----
%  RRR
% -----
@article{redal2019dynamfluid,
  title={DynamFluid: Development and Validation of a New GUI-Based CFD Tool for the Analysis of Incompressible Non-Isothermal Flows},
  author={Redal, H{\'e}ctor and Carpio, Jaime and Garc{\'\i}a-Salaberri, Pablo A and Vera, Marcos},
  journal={Processes},
  volume={7},
  number={11},
  pages={777},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{reguly2020modernising,
  title={Modernising an Industrial CFD Application},
  author={Reguly, Istv{\'a}n Z and Mudalige, Gihan R},
  booktitle={2020 Eighth International Symposium on Computing and Networking Workshops (CANDARW)},
  pages={191--196},
  year={2020},
  organization={IEEE}
}

% -----
%  SSS
% -----
@article{saad1986gmres,
  title={GMRES: A generalized minimal residual algorithm for solving nonsymmetric linear systems},
  author={Saad, Youcef and Schultz, Martin H},
  journal={SIAM Journal on scientific and statistical computing},
  volume={7},
  number={3},
  pages={856--869},
  year={1986},
  publisher={SIAM}
}

@article{sanders2020compilation,
  title={Compilation of fault-tolerant quantum heuristics for combinatorial optimization},
  author={Sanders, Yuval R and Berry, Dominic W and Costa, Pedro CS and Tessler, Louis W and Wiebe, Nathan and Gidney, Craig and Neven, Hartmut and Babbush, Ryan},
  journal={PRX Quantum},
  volume={1},
  number={2},
  pages={020312},
  year={2020},
  publisher={APS}
}

@article{scherer2017concrete,
  title={Concrete resource analysis of the quantum linear-system algorithm used to compute the electromagnetic scattering cross section of a 2D target},
  author={Scherer, Artur and Valiron, Beno{\^\i}t and Mau, Siun-Chuon and Alexander, Scott and Van den Berg, Eric and Chapuran, Thomas E},
  journal={Quantum Information Processing},
  volume={16},
  number={3},
  pages={1--65},
  year={2017},
  publisher={Springer}
}

@inproceedings{shahpar2020building,
  title={Building digital twins to simulate manufacturing variation},
  author={Shahpar, Shahrokh},
  booktitle={Turbo Expo: Power for Land, Sea, and Air},
  volume={84065},
  pages={V02AT32A049},
  year={2020},
  organization={American Society of Mechanical Engineers}
}

@article{shetty2010high,
  title={High-order incompressible large-eddy simulation of fully inhomogeneous turbulent flows},
  author={Shetty, Dinesh A and Fisher, Travis C and Chunekar, Aditya R and Frankel, Steven H},
  journal={Journal of computational physics},
  volume={229},
  number={23},
  pages={8802--8822},
  year={2010},
  publisher={Elsevier}
}

@article{smith1975comparative,
  title={Comparative study of two numerical techniques for the solution of viscous flow in a driven cavity},
  author={Smith Jr, Robert E and Kidd, Amy},
  journal={NASA Special Publication},
  volume={378},
  pages={61},
  year={1975}
}

@article{steiger2018projectq,
  title={ProjectQ: an open source software framework for quantum computing},
  author={Steiger, Damian S and H{\"a}ner, Thomas and Troyer, Matthias},
  journal={Quantum},
  volume={2},
  pages={49},
  year={2018},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}

@article{steijl2018parallel,
  title={Parallel evaluation of quantum algorithms for computational fluid dynamics},
  author={Steijl, Ren{\'e} and Barakos, George N},
  journal={Computers \& Fluids},
  volume={173},
  pages={22--28},
  year={2018},
  publisher={Elsevier}
}

@article{steijl2019quantum,
  title={Quantum algorithms for fluid simulations},
  author={Steijl, Ren{\'e}},
  journal={Advances in Quantum Communication and Information},
  pages={31},
  year={2019},
  publisher={IntechOpen}
}

@article{suau2021practical,
  title={Practical Quantum Computing: solving the wave equation using a quantum approach},
  author={Suau, Adrien and Staffelbach, Gabriel and Calandra, Henri},
  journal={ACM Transactions on Quantum Computing},
  volume={2},
  number={1},
  pages={1--35},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{suzuki1991general,
  title={General theory of fractal path integrals with applications to many-body theories and statistical physics},
  author={Suzuki, Masuo},
  journal={Journal of Mathematical Physics},
  volume={32},
  number={2},
  pages={400--407},
  year={1991},
  publisher={American Institute of Physics}
}

% -----
%  TTT
% -----
@article{trotter1959product,
  title={On the product of semi-groups of operators},
  author={Trotter, Hale F},
  journal={Proceedings of the American Mathematical Society},
  volume={10},
  number={4},
  pages={545--551},
  year={1959},
  publisher={JSTOR}
}

% -----
%  VVV
% -----
@article{vanka1985block,
  title={Block-implicit calculation of steady turbulent recirculating flows},
  author={Vanka, SP},
  journal={International journal of heat and mass transfer},
  volume={28},
  number={11},
  pages={2093--2103},
  year={1985},
  publisher={Elsevier}
}

@phdthesis{vazquez2018quantum,
  title={Quantum Algorithm for Solving Tri-Diagonal Linear Systems of Equations},
  author={V{\'a}zquez, Almudena Carrera},
  year={2018},
  school={ETH Z{\"u}rich}
}

@article{vazquez2020enhancing,
  title={Enhancing the Quantum Linear Systems Algorithm using Richardson Extrapolation},
  author={Vazquez, Almudena Carrera and Hiptmair, Ralf and Woerner, Stefan},
  journal={arXiv preprint arXiv:2009.04484},
  year={2020}
}

@book{versteeg2007introduction,
  title={An introduction to computational fluid dynamics: the finite volume method},
  author={Versteeg, Henk Kaarle and Malalasekera, Weeratunge},
  year={2007},
  publisher={Pearson education}
}

% -----
%  WWW
% -----
@book{walport2018computational,
  title={Computational Modelling: Technological Futures},
  author={Walport, M and Calder, M and Craig, C and Culley, D and de Cani, R and Donnelly, C and Douglas, R and Edmonds, B and Gascoigne, J and Gilbert, N and others},
  year={2018},
  url={https://www.gov.uk/government/publications/computational-modelling-blackett-review},
  publisher={Government Office for Science}
}

@article{wang2020quantum,
  title={Quantum fast Poisson solver: the algorithm and complete and modular circuit design},
  author={Wang, Shengbin and Wang, Zhimin and Li, Wendong and Fan, Lixin and Wei, Zhiqiang and Gu, Yongjian},
  journal={Quantum Information Processing},
  volume={19},
  number={6},
  pages={1--25},
  year={2020},
  url = {https://link.springer.com/article/10.1007/s11128-020-02669-7}
}

@article{wang2020quantumn2,
  title={A quantum Poisson solver implementable on NISQ devices},
  author={Wang, Shengbin and Wang, Zhimin and Li, Wendong and Fan, Lixin and Cui, Guolong and Wei, Zhiqiang and Gu, Yongjian},
  journal={arXiv preprint arXiv:2005.00256},
  year={2020}
}

@inproceedings{watanabe2022performance,
  title={Performance Evaluation of Lattice Boltzmann Method for Fluid Simulation on A64FX Processor and Supercomputer Fugaku},
  author={Watanabe, Seiya and Hu, Changhong},
  booktitle={International Conference on High Performance Computing in Asia-Pacific Region},
  pages={1--9},
  year={2022}
}

@article{wiebe2021theory,
  title={A Theory of Trotter Error},
  author={Wiebe, Nathan and Zhu, Shuchen},
  journal={Physical Review X},
  volume={11},
  number={011020},
  pages={26},
  year={2021}
}

% -----
%  ZZZ
% -----
@article{zhou2017efficient,
  title={Efficient quantum circuits for dense circulant and circulant like operators},
  author={Zhou, SS and Wang, JB},
  journal={Royal Society open science},
  volume={4},
  number={5},
  pages={160906},
  year={2017},
  publisher={The Royal Society Publishing}
}

